Modelling Human Mobility considering Spatial,Temporal and Social Dimensions

Modelling human mobility is crucial in several areas, from urban planning to epidemic modeling, traffic forecasting, and what-if analysis. On the one hand, existing models focus mainly on reproducing the spatial and temporal dimensions of human mobility, while the social aspect, though it influences human movements significantly, is often neglected. On the other hand, those models that capture some social aspects of human mobility have trivial and unrealistic spatial and temporal mechanisms. In this paper, we propose STS-EPR, a modeling framework that embeds mechanisms to capture the spatial, temporal, and social aspects together. Our experiments show that STS-EPR outperforms existing spatial-temporal or social models on a set of standard mobility metrics and that it can be used with a limited amount of information without any significant loss of realism. STS-EPR, which is open-source and tested on open data, is a step towards the design of mechanistic models that can capture all the aspects of human mobility in a comprehensive way.

==> chapter_3_other_models.tex <==
\subsection{GeoSim}\label{sect:geosim}
GeoSim, proposed by Toole et al. \cite{geosim}, extends the EPR model presented by Song et al. \cite{im_model_song}.
The EPR model considers only the spatial and temporal dimensions during the generation of the synthetic trajectories.
GeoSim, instead, takes into account also the social dimension to model the fact that about $10$-$30\%$ of the human movements can be explained by social purposes \cite{cho}.
GeoSim introduces two mechanisms in addition to the presented ones: individual preference and social influence.
When an agent decides to explore or return, it has to determine if the choice will be affected or not by the other agents, with a probability, respectively, of $\alpha$ and $1-\alpha$, where $\alpha=0.2$ is a constant \cite{geosim}.
In the individual preference mechanism, the agent behaves selecting the location according to its visitation pattern, without any influences of the other agents involved.
Otherwise, in the social influence mechanism, an agent selects the location to explore or return with the influence of the visitation patterns of its social contacts (i.e., a user $i$ is a social contact for $u$ if exists an edge $(u,i)$ in the social graph).

The model takes in input:
\begin{itemize}
    \item $N$: the number of synthetic individuals;
    \item $L$: a tessellation of the space where the agents are allowed to move;
    \item $G$: an undirected graph modeling the sociality of the $N$ agents;
    \item $min_{wt}$: the minimum amount of time an agent spend in a location, set to 1 hour;
    \item $[start, end]$: the time interval of the simulation;
\end{itemize}{}
and outputs the generated synthetic trajectories.

GeoSim can be decomposed into three phases: initialization, action selection and location selection.

In the initialization phase, a set of $N$ agents are distributed randomly across $|L|$ locations and connected in an undirected graph, called social graph, describing the social links between agents. 
The weight corresponding to each edge represents the mobility similarity between the linked agents.
The location vector $lv$ of each agent is initialized to reflect its single visit, and the number $S$ of visited locations is set to one.
At the end of this phase, each agent selects a waiting time $\Delta t \geq min_{wt}$ from the empirical probability density function $P(\Delta_t) \approx \Delta_t^{-\beta} e^{-\Delta_t / \tau}$ \cite{im_model_song}; each agent is allowed to move after the picked $\Delta t$.

After the initialization phase, every agent decides whether or not to move according to its own waiting time.
When an agent moves, performs the action and location selection steps, then chooses a new waiting time, updates the location vector and, if the agent explored a new location, $S$ is incremented by one.
The agents iterates these actions until a stopping criterion is satisfied (e.g., the number of hours to simulate is reached).

During the action selection phase (Figure \ref{fig:action_schema}), the agent first chooses to either visit a new location with probability $P_{exp}=\rho S^{-\gamma}$ or to return to a previously visited location with probability $P_{ret}=1-\rho S^{-\gamma}$. At that point, independently of the mechanisms selected, the agent chooses to perform the location selection phase individually with probability $1-\alpha$ or with the influence of its contacts with probability $\alpha$.

After the agent picked the action among the four combinations, in the location selection phase the agent selects the destination of its move according to the chosen mechanisms.
For an agent $a$, we define the sets containing the indices of the locations $a$ can explore or return respectively, as follows:
\begin{equation}\label{equation:set_exp}
    exp_a = \{i\;|\;lv_a[i]=0\}
\end{equation}
\begin{equation}
    ret_a = \{i\;|\;lv_a[i] > 0\}
\end{equation}\label{equation:set_ret}
The frequency of visits of an individual $a$ relative to a location $r_i$ is referred as $f_a(r_i)$.


\begin{itemize}
    \item \textbf{Exploration-Individual:}  During the individual exploration, an agent $a$ chooses a new location to explore from the set $exp_a$ uniformly at random.
    The probabiliy $p(r_i)$ for a location $r_i$ with $i\in exp_a$ to be selected is $\frac{1}{|exp_a|}$.
    \item \textbf{Exploration-Social:} In the social exploration action, an agent $a$ selects a social contact $c$.
    The probability $p(c)$ for a social contact $c$ to be selected is directly proportional to the mobility-similarity between them: $p(c) \propto mob_{sim}(a,c)$.
    After the contact $c$ is chosen, the location to explore is selected from the set $A = exp_a \cap ret_c$; the probability $p(r_i)$ for a location $r_i$, with $i\in A$, to be selected is proportional to the visitation pattern of the agent $c$, namely $p(r_i) \propto f_c(r_i)$.
    \item \textbf{Return-Individual:} In the individual return action, an agent $a$ picks the return location from the set $ret_a$ with a probability directly proportional to its visitation pattern.
    The probability for a location $r_i$ with $i\in ret_a$ to be chosen is: $p(r_i) \propto f_a(r_i)$.
    \item \textbf{Return-Social:} The contact $c$ is selected as in the Exploration-Social action, while the set where the location is selected from is defined as $A = ret_a \cap ret_c$; the probability $p(r_i)$ for a location $r_i$ to be selected is proportional to the visitation pattern of the agent $c$, namely $p(r_i) \propto f_c(r_i)$.
\end{itemize}{}

\begin{figure}
    \centering
    \begin{tikzpicture}[level distance=2.5cm,
      level 1/.style={sibling distance=5cm},
      level 2/.style={sibling distance=2.5cm}]
      \node {agent moves}
        child {node {explore}
          child {node {individual} edge from parent node [left] {$1-\alpha \;$}}
          child {node {social} edge from parent node [right] {$\; \alpha$}}
           edge from parent node [left] {$\rho S^{-\gamma} \;$}
        }
        child {node {return}
        child {node {individual} edge from parent node [left] {$1-\alpha \;$}}
          child {node {social} edge from parent node [right] {$\; \alpha$}}
          edge from parent node [right] {$\; 1-\rho S^{-\gamma}$}
        };
    \end{tikzpicture}
    \caption[Action selection phase of GeoSim and its extensions]{A schematic description of the action selection phase of the considered models. 
    The individual first decides whether to explore a new location or return to a previously visited one.
    Then the agent determines if its social contacts will affect or not its choice for the location to visit next.}
    \label{fig:action_schema}
\end{figure}

\subsection{GeoSim-distance}\label{sect:gs_d}
A modeling limit of GeoSim concerns the spatial patterns of the generated synthetic trajectories.
GeoSim does not take into account the distance from the current location and the location to explore \cite{geosim}, since the destination of the next move is chosen uniformly at random.
Consequently, the probability density functions for both jump size and radius of gyration of the generated trajectories do not follow the proper empirical distribution \cite{gonzalez_understanding}.

The power-law behavior of the probability density function of the jump length suggests that individuals are more likely to move at small rather than long distances. To take into account this observation in the first extension of GeoSim, namely $\mbox{GS}_d$, in the Exploration-Individual action an agent $a$ currently at location $r_j$, selects an unvisited location $r_i$, with $i \in exp_a$, with probability $p(r_i)\propto \frac{1}{d_{ij}}$ where $d_{ij}$ is the geographic distance between location $r_i$ and $r_j$.

\subsection{GeoSim-gravity}\label{sect:gs_gravity}
Individuals do not consider the distance from a place as the only discriminant factor while selecting the next location to explore.
They are driven by a preferential-exploration force in the selection of the new location to explore \cite{d_epr,ditras}.
The individuals take into account also the relevance of a location at a collective level together with the distance from their current location.
The method used for coupling both the distance and the relevance is the same used in the \textit{d-EPR} model \cite{d_epr}: the use of a gravity law.
The usage of the gravity model is justified by the accuracy of the gravity model to estimate origin-destination matrices even at the country level \cite{d_epr}.

In $\mbox{GS}_{gravity}$, the second proposed extension of GeoSim, an agent $a$ currently at location $r_j$, during the Exploration-Individual action  selects an unvisited location $r_i$, with $i \in exp_a$, with probability $p(r_i)\propto \frac{w_i w_j}{d_{ij}^2}$ where $d_{ij}$ is the geographic distance between location $r_i$ and $r_j$ and $w_i$, $w_j$ represent their relevance.

The relevance of a location can be estimated through the measure visits per location (Sect. \ref{sect:measures}), using a real mobility dataset. In case the real information is not available, the relevance of a location can be estimated using the population density \cite{ditras}.

\subsection{GeoSim-diary}\label{sect:gs_diary}
Both the proposed extensions focus on the improvement of the spatial patterns of the generated trajectories.
As discussed before, the displacements of human beings follow a circadian rhythm since individuals are mainly stationary during the night and move at a specific time of the day \cite{ditras,opp_net}.
In the discussed models is not included any mechanism able to capture the individual's recurrent and periodic schedules. in fact the periodicity of the displacement of an individual is given from its waiting times. 

To model the individuals' routines, we propose $\mbox{GS}_{diary}$, an extension of GeoSim; in $\mbox{GS}_{diary}$, we use a mobility diary generator, an algorithm able to capture the tendency of individuals to follow or break their routine \cite{ditras}.
During the first step, the model assigns at each agent a mobility diary produced by the mobility generator.
A mobility diary $\mbox{MD}$ for an agent $a$ is defined as:
\begin{equation}
    \mbox{MD}_a = \langle (ab_0,t_1), (ab_1,t_2), \dots (ab_j,t_{j+1}), (ab_0,t_{j+2}), \dots)\rangle
\end{equation}{}
Where $ab$ is an \textit{abstract location}, $ab_0$ denotes the home location of the agent $a$ and the visits between two home locations are called $run$.
The abstract location $ab_0$ is assigned randomly to a physical location in the initialization step.

The agent will move according to the entries in its mobility diary: if the current abstract location is $ab_0$ the agent visits the home location, otherwise converts the abstract location into a physical one selecting the location to visit with the same approach as in $\mbox{GS}_{gravity}$. 
The physical locations visited by an individual during a run must be distinct from each other, but the physical location resulting from the  mapping of $ab_i$ can be different in different runs.
In $\mbox{GS}_{diary}$ there is no need to select a waiting time from the empirical distribution \cite{song_limits}, since it is intrinsically specified in the mobility diary.


\subsection{Additional features}\label{sect:additional}
For each of the presented models, we introduce some additional features that may capture in a realistic way some crucial aspects of human mobility.

\subsection*{Relevance-based Starting Locations}\label{sect:rsl}
Given a weighted spatial tessellation $L$, during the initialization phase, the agents are assigned to a starting location $r_i$ with a probability $p(r_i) \propto \frac{1}{|L|}$.
With the introduction of the concept of relevance at a collective level for a location, we decide to propose a new strategy for assigning the agents at the starting location, the RSL (Relevance-based Starting Locations).
In this strategy the agents aren't assigned uniformly at random, the probability $p(r_i)$ for an agent of being assigned to a starting location $r_i$ is $\propto w_i$, where $w_i$ is the relevance of the location at a collective level.


\subsection*{Reachable locations}\label{sect:reachable}
When a synthetic individual is allowed to move, it is associated with a waiting time, extracted from the empirical distribution $P(\Delta_t) \approx \Delta_t^{-\beta} e^{-\Delta_t / \tau}$ \cite{im_model_song}, or specified in the mobility diary of the agent, depending on which extension of GeoSim in considered.
The agent associated with a waiting time $\Delta_t$ can not physically visit every location, but realistically only the locations the individual can reach moving at a certain speed for the picked amount of time.

We define $speed_{agent}$ as the typical speed of an individual and $I$ as the set of all the locations the agent can visit, the set $R$ of the reachable locations for an agent starting from the location $r_j$ is computed as follows:
\begin{equation}
    R = \{i \in I\;|\;dist(r_j,r_i) \leq dist_{max}\}
\end{equation}\label{equation:reachable}
where $dist_{max}= \Delta t \cdot speed_{agent}$

\subsection*{Social Choice by Degree}\label{sect:by_degree}
When an agent $a$ performs a social action, selects a contact $c$ with a probability $p(c) \propto mob_{sim}(a,c)$.
The choice of the social contact is personal for the agent; in fact, it is determined using only individual information, and no collective information is considered.
We propose a new contact selection method.
During a social return, the selection process is the same as the presented models.
Instead, in the social exploration, the contact is determined using its popularity at the collective level.
The popularity $pop$ of an individual $u$ within a social graph $G$ is defined as:
\begin{equation}
    pop(u,G) = deg(u,G)
\end{equation}{}
where the degree of a node $n$ in the graph $G$ is denoted as $deg(n,G)$.
In the social exploration, an agent $a$ selects a social contact $c$ with probability $p(c) \propto pop(c,G)$.

The intuition underlying this proposal is very simple.
When an individual decides to explore a new location with the influence of a contact, a popular contact will be more likely to influence its decision than an unpopular one, even if their mobility patterns are very different.
For example, an event promoter (generally a popular node within a social graph) has a high probability of influencing the choice of one of its contacts, during the selection of the next location to explore, even though they can have different mobility behaviors.
In contrast, when an individual decides to return at an already visited location with the influence of its social contacts, it is reasonable to think that the choice of the contact is conducted using individual information.
During the return action, individuals follow their routine, consequently they are more likely to select a contact with a similar mobility pattern.



\subsection*{Action-correction phase}
The location an agent can select as the destination of its next displacement is constrained.
In several cases, the set of locations where the individual is allowed to move is empty; in the literature, it is unspecified how to deal with these situations.
We extend the models including a new phase: the action correction phase. The action correction phase is executed after the location selection, if the latter is too restrictive and do not allow movements in any location.

\begin{itemize}
    \item \textbf{No new location to explore}: When an individual $a$ performs the selection action phase (Figure \ref{fig:action_schema}) and decides to explore individually an unvisited location, it selects the location from the set $exp_a$ (Equation \ref{equation:set_exp}).
    In case the individual visited all the locations at least one time, no choice can be made since $exp_a=\varnothing$.
    We deal with this case correcting the action (Figure \ref{fig:routine_1}) of the individual from Exploration-Individual to Return-Individual, preserving in this way the choice of performing the location selection without any influence of its social contacts.
    \item \textbf{No location in social choices}: If the agent $a$ decide to move with the influence of a social contact $c$, and the set $A$ computed for the relative action $A = ret_a \cap ret_c$ or $A = exp_a \cap ret_c$ is empty, we correct the action from the current to Return-Individual (Figure \ref{fig:routine_1}).
    \item \textbf{No reachable locations}: When a synthetic individual is allowed to move, it is associated with a waiting time $\Delta t$, and it can reach the locations in the set $R$ (Eq. \ref{equation:reachable}).
    The set $R$ may be empty even if $I\neq\varnothing$, meaning there is no location the agent can visit within the radius $dist_{max}$ but the set of possible choices is not empty.
    If the agent was performing an exploration, a new $\Delta t_1 > \Delta t$ is selected to expand the area the agent can cover during its displacement. After picking the new waiting time the set $R$ is computed, if $R=\varnothing$ then a new $\Delta t_2 > \Delta t_1$ is picked, (this procedure is repeated for a maximum of $n_{max}$ time) and an Exploration-Individual action is performed with the new waiting time.
    If the agent was performing a Return-Social action or in the case the incrementing of the waiting time was performed $n_{max}$ times, then the action is corrected with a Return-Individual; note that Return-Individual can not fail, since the agent can always return in its current location $r_j$ from the moment that $dist(r_j,r_j)=0$ (Figure \ref{fig:routine_2}).
    \item \textbf{Run in the Mobility Diary}: In the mobility diary the locations visited by an individual during a \textit{run} (defined as the visits between two home return) must be distinct from each other.
    Given a run $d=\langle ab_1, ab_2, \dots , ab_n \rangle$ of length $n$, all the abstract locations $ab_i \in d$ must be assigned to distinct physical locations, the mapping between the abstract locations in $d$ and the real locations in $L$ must be injective.
    The injectivity of the mapping can not always be guaranteed: the location selection can fail due to the three cases presented above. 
    With the use of the mobility diary, also the Individual-Return action can fail, since the agent can not even visit its current location.\\
    In the action correction phase (Figure \ref{fig:routine_3}), if a social choice can not be completed, the next action executed is the action with the same mechanism performed without the influence of social contacts. In the case an individual action can not be performed, the complementary individual action is performed.
    If even the complementary individual action fails, the agent returns to the home location..
    When an agent returns to the home location due to action failure during the assignment of the abstract location $ab_j \in d$, the run $d$ is splitted in $d1=\langle ab_1,\dots,ab_j \rangle$, $d2=\langle ab_{j+1},\dots,ab_n \rangle$ and the agent start the mapping of the new run $d2$.
\end{itemize}{}



\begin{figure}
    \centering
    \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp5113533713537675] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.39 ][line width=0.75]  (28,28.17) -- (173,28.17) -- (173,53.17) -- (28,53.17) -- cycle ;
%Shape: Rectangle [id:dp2453357910618561] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.39 ][line width=0.75]  (28,104.25) -- (173,104.25) -- (173,129.25) -- (28,129.25) -- cycle ;
%Shape: Rectangle [id:dp7554144177886372] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.39 ][line width=0.75]  (28,180.33) -- (173,180.33) -- (173,205.33) -- (28,205.33) -- cycle ;
%Shape: Rectangle [id:dp22357315421503277] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.24 ][line width=0.75]  (276.75,104.2) -- (421.75,104.2) -- (421.75,129.2) -- (276.75,129.2) -- cycle ;
%Straight Lines [id:da605229715687423] 
\draw    (172.6,117) -- (273.8,116.81) ;
\draw [shift={(276.8,116.8)}, rotate = 539.89] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da8764141750437828] 
\draw    (172.9,193.1) .. controls (263.57,192.17) and (307.81,184.51) .. (329.19,173.85) .. controls (349.18,163.87) and (348.45,146.62) .. (348.27,132.52) ;
\draw [shift={(348.25,129.63)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da4489926881144929] 
\draw    (172.9,39.86) .. controls (263.57,40.79) and (307.81,48.45) .. (329.19,59.11) .. controls (349.18,69.08) and (348.45,86.33) .. (348.27,100.44) ;
\draw [shift={(348.25,103.33)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da7321976587724227] 
\draw    (419,46) -- (472,46) ;
\draw [shift={(475,46)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

% Text Node
\draw (424,31) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {if fails};
% Text Node
\draw  [draw opacity=0]  (298.75,105.25) -- (399.75,105.25) -- (399.75,128.25) -- (298.75,128.25) -- cycle  ;
\draw (349.25,109.25) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Return-Individual}};
% Text Node
\draw  [draw opacity=0]  (59,181.38) -- (142,181.38) -- (142,204.38) -- (59,204.38) -- cycle  ;
\draw (100.5,185.38) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Return-Social}};
% Text Node
\draw  [draw opacity=0]  (38,29.22) -- (163,29.22) -- (163,52.22) -- (38,52.22) -- cycle  ;
\draw (100.5,33.22) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Exploration-Individual}};
% Text Node
\draw  [draw opacity=0]  (47,105.3) -- (154,105.3) -- (154,128.3) -- (47,128.3) -- cycle  ;
\draw (100.5,109.3) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Exploration-Social}};


\end{tikzpicture}
    \caption[Action correction phase of GeoSim for handling cases where the agent can neither explore nor perform a social choice]{A description of the action correction routine in the case the agent can neither explore nor perform a social choice.
    The green rectangle denotes a starting state while the light blue a final state.
    When one of the already mentioned action fails, a Return-Individual is executed; the individual return at an already visited location can always be performed since the set $ret_a$ contains always at least one element, the starting location of the individual.}
    \label{fig:routine_1}
\end{figure}{}


\begin{figure}
    \centering
    \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp974259444763385] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.39 ][line width=0.75]  (39,89.17) -- (184,89.17) -- (184,114.17) -- (39,114.17) -- cycle ;
%Shape: Rectangle [id:dp1457414964556758] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.39 ][line width=0.75]  (39,165.25) -- (184,165.25) -- (184,190.25) -- (39,190.25) -- cycle ;
%Shape: Rectangle [id:dp8480688434708062] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.39 ][line width=0.75]  (39,241.33) -- (184,241.33) -- (184,266.33) -- (39,266.33) -- cycle ;
%Shape: Rectangle [id:dp9823103326517663] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.24 ][line width=0.75]  (236,127.21) -- (381,127.21) -- (381,152.21) -- (236,152.21) -- cycle ;
%Straight Lines [id:da22512986954348035] 
\draw    (452,89) -- (505,89) ;
\draw [shift={(508,89)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Rectangle [id:dp10096827047725765] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.24 ][line width=0.75]  (362,192.29) -- (507,192.29) -- (507,217.29) -- (362,217.29) -- cycle ;
%Curve Lines [id:da6487326705019393] 
\draw    (184,178.33) .. controls (221.29,178.29) and (172.78,140.86) .. (232.53,139.69) ;
\draw [shift={(235.33,139.67)}, rotate = 539.96] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da7976095260803209] 
\draw    (381.4,139.6) .. controls (431.49,86.04) and (310.66,37.77) .. (309.01,124.53) ;
\draw [shift={(309,127.2)}, rotate = 269.49] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da2389580348633935] 
\draw    (381.4,140) .. controls (441.77,139.22) and (434.14,144.19) .. (433.81,188.82) ;
\draw [shift={(433.8,191.6)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da7182631436364411] 
\draw    (184.6,254.4) .. controls (276.54,254.8) and (252.05,204.9) .. (359.77,204.8) ;
\draw [shift={(361.4,204.8)}, rotate = 180.21] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da6336276610279128] 
\draw    (184,101) .. controls (221.29,101.05) and (172.78,138.47) .. (232.53,139.64) ;
\draw [shift={(235.33,139.67)}, rotate = 180.04] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

% Text Node
\draw (457,74) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {if fails};
% Text Node
\draw  [draw opacity=0]  (384,193.34) -- (485,193.34) -- (485,216.34) -- (384,216.34) -- cycle  ;
\draw (434.5,197.34) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Return-Individual}};
% Text Node
\draw  [draw opacity=0]  (70,242.38) -- (153,242.38) -- (153,265.38) -- (70,265.38) -- cycle  ;
\draw (111.5,246.38) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Return-Social}};
% Text Node
\draw  [draw opacity=0]  (49,90.22) -- (174,90.22) -- (174,113.22) -- (49,113.22) -- cycle  ;
\draw (111.5,94.22) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Exploration-Individual}};
% Text Node
\draw  [draw opacity=0]  (58,166.3) -- (165,166.3) -- (165,189.3) -- (58,189.3) -- cycle  ;
\draw (111.5,170.3) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Exploration-Social}};
% Text Node
\draw  [draw opacity=0]  (246,128.26) -- (371,128.26) -- (371,151.26) -- (246,151.26) -- cycle  ;
\draw (308.5,132.26) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Exploration-Individual}};
% Text Node
\draw (41,117.17) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize \textit{i = 0}}};
% Text Node
\draw (41,193.25) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize \textit{i = 0}}};
% Text Node
\draw (238,155.21) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize \textit{i++}}};
% Text Node
\draw (256,60.21) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize \textit{if i }$\displaystyle \leq $\textit{ n\_max}}\\ \ \ {\footnotesize \textit{pick} $\displaystyle \Delta t$}};
% Text Node
\draw (439,153.21) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize \textit{if i }$\displaystyle  >$\textit{ n\_max}}};


\end{tikzpicture}

    \caption[The action correction routine for handling cases where the agent can not reach any of the possible locations]{In the action correction routine designed for handling cases where the agent can not reach any of the possible locations, if the individual was performing an exploration action a new waiting time, greater than the current one, is picked; if it still can not reach any location the latter procedure is repeated at most $n_{max}$ times. If the agent was performing a Return-Social action or after $n_{max}$ increments, the action is corrected with a Return-Individual; Return-Individual can always be performed since the agent can return in its current location $r_j$ from the moment that $dist(r_j,r_j)=0$.}
    \label{fig:routine_2}
\end{figure}{}


\begin{figure}
    \centering
    

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp9834864376310755] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.39 ][line width=0.75]  (5,25.33) -- (150,25.33) -- (150,50.33) -- (5,50.33) -- cycle ;
%Shape: Rectangle [id:dp7477956579662924] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.39 ][line width=0.75]  (5,252.25) -- (150,252.25) -- (150,277.25) -- (5,277.25) -- cycle ;
%Shape: Rectangle [id:dp06197678997697065] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.39 ][line width=0.75]  (57,202.17) -- (202,202.17) -- (202,227.17) -- (57,227.17) -- cycle ;
%Shape: Rectangle [id:dp5471962864909669] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.39 ][line width=0.75]  (57,75.17) -- (202,75.17) -- (202,100.17) -- (57,100.17) -- cycle ;
%Shape: Rectangle [id:dp4894812552173363] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.24 ][line width=0.75]  (242,75.17) -- (387,75.17) -- (387,100.17) -- (242,100.17) -- cycle ;
%Shape: Rectangle [id:dp08769918989632797] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.24 ][line width=0.75]  (242,202.17) -- (387,202.17) -- (387,227.17) -- (242,227.17) -- cycle ;
%Straight Lines [id:da0223920854812919] 
\draw    (202.51,88.2) -- (238,88.2) ;
\draw [shift={(241,88.2)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da4573560195403087] 
\draw    (202.2,214.4) -- (237.69,214.4) ;
\draw [shift={(240.69,214.4)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da008506612234683963] 
\draw    (24.33,252.17) .. controls (23.75,209.87) and (23.42,213.91) .. (52.24,214.46) ;
\draw [shift={(55,214.5)}, rotate = 180.54] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da18109780648993323] 
\draw    (24.33,50.33) .. controls (23.75,92.63) and (23.42,88.59) .. (52.24,88.04) ;
\draw [shift={(55,88)}, rotate = 539.46] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Rectangle [id:dp6222145563005488] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.24 ][line width=0.75]  (347,138.17) -- (492,138.17) -- (492,163.17) -- (347,163.17) -- cycle ;
%Curve Lines [id:da3793029739915291] 
\draw    (387.57,87.71) .. controls (426.21,86.33) and (419.3,91.68) .. (419.76,135.28) ;
\draw [shift={(419.8,138)}, rotate = 269.01] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da2704480948483904] 
\draw    (387.57,214.81) .. controls (426.21,216.2) and (419.3,210.85) .. (419.76,167.24) ;
\draw [shift={(419.8,164.53)}, rotate = 450.99] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da9968386004676839] 
\draw    (429,35) -- (482,35) ;
\draw [shift={(485,35)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

% Text Node
\draw  [draw opacity=0]  (36,26.38) -- (119,26.38) -- (119,49.38) -- (36,49.38) -- cycle  ;
\draw (77.5,30.38) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Return-Social}};
% Text Node
\draw  [draw opacity=0]  (24,253.3) -- (131,253.3) -- (131,276.3) -- (24,276.3) -- cycle  ;
\draw (77.5,257.3) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Exploration-Social}};
% Text Node
\draw  [draw opacity=0]  (67,203.22) -- (192,203.22) -- (192,226.22) -- (67,226.22) -- cycle  ;
\draw (129.5,207.22) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Exploration-Individual}};
% Text Node
\draw  [draw opacity=0]  (79,76.22) -- (180,76.22) -- (180,99.22) -- (79,99.22) -- cycle  ;
\draw (129.5,80.22) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Return-Individual}};
% Text Node
\draw  [draw opacity=0]  (252,76.22) -- (377,76.22) -- (377,99.22) -- (252,99.22) -- cycle  ;
\draw (314.5,80.22) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Exploration-Individual}};
% Text Node
\draw  [draw opacity=0]  (264,203.22) -- (365,203.22) -- (365,226.22) -- (264,226.22) -- cycle  ;
\draw (314.5,207.22) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Return-Individual}};
% Text Node
\draw  [draw opacity=0]  (373.5,139.22) -- (465.5,139.22) -- (465.5,162.22) -- (373.5,162.22) -- cycle  ;
\draw (419.5,143.22) node [anchor=north] [inner sep=0.75pt]  [font=\small] [align=left] {{\small Home Location}};
% Text Node
\draw (434,20) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {if fails};


\end{tikzpicture}

    \caption[The action correction routine for guarantee the injective mapping of the abstract location visited during a run]{In the action correction routine, in order to guarantee the injective mapping of the abstract location visited during a run, if the agent was executing a social choice the action is corrected in an individual one, preserving the mechanism selected. If an individual action can not be performed the complementary one is executed, if it fails then the agent returns home.}
    \label{fig:routine_3}
\end{figure}{}

\subsection{Implementation}\label{sect:implementation}
We implement GeoSim and the presented extension in \texttt{GeoSim}, a \texttt{Python} open source algorithm for generating realistic mobility trajectories \footnote{The Python source code of \texttt{GeoSim} is freely available for download at \href{https://github.com/kdd-lab/2019_Cornacchia}{https://github.com/kdd-lab/2019\_Cornacchia}}.
\texttt{GeoSim} is build using the mobility structure of \texttt{scikit-mobility} \cite{scikit_mobility}.

\subsection*{Parameters}
The main class, \texttt{GeoSim}, takes several parameters in input; they can be classified into four categories:

\begin{itemize}
    \item \textbf{distributions}: The parameters in this category defines the constants used in the model. The constants $\rho$ and $\gamma$ affect the probability for an individual to return or explore, $\alpha$ corresponds at the social factor, namely the probability of being influenced by a social contact in the choice of the next displacement, $\tau$ and $min\_wt\_hours$ are the constants used in the waiting time distribution.
    The default values for the constants are reported in Table \ref{tab:table_constants}.
    \item \textbf{simulation}: The parameters in this category specifies the number \texttt{n\_agents} of agents to simulate, the extremes of the time interval to simulate, respectively \texttt{start\_date} and \texttt{end\_date}; the parameter \texttt{social\_graph} if specified is interpreted as the edge list of the social graph and the weighted spatial tessellation is specified in the parameter \texttt{spatial\_tessellation}.
    \item \textbf{model}: The combinations of the values of the parameters in this group define which one of the presented generative models will be executed (Table \ref{tab:table_models_gs}). The boolean parameter \texttt{distance} defines if the models will use the distance as a factor in the location selection, \texttt{gravity} indicates if the model will use the gravity law in the selection of the destination of the next displacement of an individual, and the parameter \texttt{diary\_generator}, if specified, denotes a \texttt{MarkovDiaryGenerator} object which represents the mobility diary generator, the model will use it generate the mobility diary for each agent.
    \item \textbf{additional features}: The parameters in this category control the additional features used in the execution;
    the boolean parameter \texttt{rsl} defines whether or not agent are assigned to a starting location with probability proportional to the relevance of a location or uniformly at random, the parameter \texttt{max\_speed\_km\_h}, if specified, indicates the typical speed $speed_{agent}$ of the agents, the boolean parameter \texttt{degree\_exp\_social} defines if during the social exploration the is chosen proportionally to its degree or not.
    
\end{itemize}{}



\begin{table}
    \centering
    \begin{tabular}{l|cccccc}
    \textbf{parameter} & \texttt{rho} & \texttt{gamma} & \texttt{alpha} & \texttt{beta} & \texttt{tau} & \texttt{min\_wt\_hours} \\ \hline
    \textbf{value}     & 0.6 & 0.21  & 0.2   & 0.8  & 17  & 1                     
    \end{tabular}
    \caption[The default values of the distributions' parameters]{The default values of the distributions' parameters.}
    \label{tab:table_constants}
\end{table}


\begin{table}
\centering
\begin{tabular}{l|ccc}
models                & \texttt{distance} & \texttt{gravity} & \texttt{diary\_generator} \\ \hline
GeoSim                & False    & False   & None             \\
$\mbox{GS}_{d}$       & True     & False   & None             \\
$\mbox{GS}_{gravity}$ & True     & True    & None             \\
$\mbox{GS}_{diary}$   & True     & True    & mobility\_diary 
\end{tabular}
\caption[The different combinations of the models' parameter for each presented model]{The different combinations of the models' parameter for each presented model.}
\label{tab:table_models_gs}
\end{table}


\subsection*{Data Structures}
The most important data structures used for modelling efficiently the different aspects of the human mobility are the following:
\begin{itemize}
    \item \textbf{Mobility Pattern}: The visitation pattern $lv_a$ of an agent $a$ is modeled as a vector of $|L|$ elements, where $|L|$ it the total number of locations.
    \item \textbf{Distance Matrix}:  The distance matrix $D$ is a square matrix of dimension $|L|\times|L|$ where $|L|$ is the total number of locations. Each entry $d_{ij} \in D$ contains the spatial distance in km between location $r_i$ and location $r_j$. For optimizing the space used by the process, the matrix is represented in memory as a sparse matrix, and it is populated only when necessary.
    \item \textbf{Trajectories}: the trajectories generated by the model are described by a \texttt{TrajDataFrame}, a data structure of the library scikit-mobility \cite{scikit_mobility}; it contains the user identifier, the coordinates of the location and a timestamp.
    \item \textbf{Spatial Tessellation}: the spatial tessellation is represented through a \texttt{DataFrame}, containing for each location its identifier, the coordinates and the relevance at a collective level.
\end{itemize}



\subsection*{Time complexity}

In the initialization phase, the agents are assigned randomly to a home location, this procedure costs $\mathcal{O}(n)$, where $n$ is the number of agents in the simulation.
In the worst case scenario, each of the $n$ agents move every $min_{wt}$ hours, performing $m=\frac{total_h}{min_{wt}}$ movements, where $total_h$ corresponds at the number of hours simulated; consequently the number of actions performed in the simulation is $O(n\cdot m)$, in each action selection phase the agent generates at most four random numbers, each generation costs $\mathcal{O}(1)$ and during the location selection phase the model iterates through the location vector $\mathcal{O}(L)$ in order to build the set of the locations the agent can visit.
In the case all the locations are visited at least one time, all the entries in the distance matrix $M$ are computed, this operation costs $\mathcal{O}(L^2)$.
The time complexity of the proposed implementation is $\approx \mathcal{O}(n + 4nm + Lnm + L^2)$.

\subsection*{Example of execution}

The following code shows how to simulate the mobility of 50 agents connected in a social graph given a weighted spatial tessellation during an observation period of three months.
The choice of the parameters instantiate the model $\mbox{GS}_{gravity}$, as shown in Table \ref{tab:table_models_gs}.

\vspace{1cm}

\begin{lstlisting}[language=Python, basicstyle=\footnotesize\ttfamily]
import GeoSim as gs

#load a weighted spatial tessellation
tex = pickle.load(open("tessellation_250m.pickle","rb"))

#load a social graph of 50 individuals (edge list)
graph = pickle.load(open("social_graph_50_agents.pickle","rb"))

# define the period of the simulation
start_date = pandas.to_datetime("2012/04/10 00:00:00")
end_date = pandas.to_datetime("2012/07/10 00:00:00")

#create a new istance of GeoSim
geosim = gs.GeoSim()

#generate the synthetic trajectories with the specified parameters
tdf = geosim.generate(start_date, end_date, n_agents = 50,
                    spatial_tessellation = tex, rsl = True, 
                    distance = True, gravity = True, 
                    social_graph = graph)


\end{lstlisting}
\vspace{1cm}

The output of the method \texttt{geosim.generate} is a \texttt{TrajDataFrame} that contains the simulated displacements made by the agents.
Each record in the \texttt{TrajDataFrame} contains a user identifier, a timestamp corresponding at the time of the displacement and the coordinates of the visited location; an example of the output generated by the model is shown in Table \ref{tab:tdf}.
The output in sorted in ascending order by \texttt{uid} and \texttt{timestamp}.


\begin{table}[H]
\renewcommand*{\arraystretch}{1.2}
    \centering
\begin{tabular}{ccccc}
\hline
 &
  \texttt{uid} &
  \texttt{lat} &
  \texttt{lng} &
  \texttt{timestamp} \\ \hline
{\color[HTML]{000000} \textbf{0}} &
  {\color[HTML]{000000} 19} &
  {\color[HTML]{000000} 40.734004} &
  {\color[HTML]{000000} -73.988473} &
  {\color[HTML]{000000} 2012-04-10 00:00:00.000000} \\
{\color[HTML]{000000} \textbf{1}} &
  {\color[HTML]{000000} 19} &
  {\color[HTML]{000000} 40.734004} &
  {\color[HTML]{000000} -73.988473} &
  {\color[HTML]{000000} 2012-04-10 03:29:57.112640} \\
{\color[HTML]{000000} \textbf{2}} &
  {\color[HTML]{000000} 19} &
  {\color[HTML]{000000} 40.734004} &
  {\color[HTML]{000000} -73.988473} &
  {\color[HTML]{000000} 2012-04-10 08:34:19.532325} \\
{\color[HTML]{000000} \textbf{3}} &
  {\color[HTML]{000000} 19} &
  {\color[HTML]{000000} 40.713580} &
  {\color[HTML]{000000} -73.950294} &
  {\color[HTML]{000000} 2012-04-10 21:38:10.585138} \\
{\color[HTML]{000000} \textbf{4}} &
  {\color[HTML]{000000} 19} &
  {\color[HTML]{000000} 40.734004} &
  {\color[HTML]{000000} -73.988473} &
  {\color[HTML]{000000} 2012-04-11 01:21:49.630914} \\
$\vdots$ &
  $\vdots$ &
  $\vdots$ &
  $\vdots$ &
  $\vdots$
\end{tabular}
    \caption[An example of a \texttt{TrajDataFrame} structure containing the generated trajectories]{An example of a \texttt{TrajDataFrame} structure containing the generated trajectories.
    Each record contains a user identifier \texttt{uid}, the timestamp corresponding at the synthetic displacement \texttt{timestamp}
    and the coordinates of the visited location \texttt{lat} and \texttt{lng}.}
    \label{tab:tdf}
\end{table}{}




The class \texttt{GeoSim} uses the structure of the library \textit{scikit-mobility} and could be easily merged in that framework.
The constructor method \texttt{GeoSim()} instantiate a new object; it takes as parameters the distribution's parameters (the default values are shown in Table \ref{tab:table_constants}).
The method \texttt{generate()} takes in input the parameters in the categories simulation, model and additional features; it outputs a \texttt{TrajDataFrame} containing the generated trajectories of the agents.
Through a \texttt{GeoSim} object is possible to access at the attribute \texttt{social\_graph} containing a representation of the social graph used in the simulation, and at the attribute \texttt{agents} containing the information of the agents (e.g., location vector, starting position and number of distinct locations visited).




